Almost Optimal Tensor Sketch

We construct a matrix $M\in R^{m\otimes d^c}$ with just $m=O(c\,\lambda\,\varepsilon^{-2}\text{poly}\log1/\varepsilon\delta)$ rows, which preserves the norm $\|Mx\|_2=(1\pm\varepsilon)\|x\|_2$ of all $x$ in any given $\lambda$ dimensional subspace of $ R^d$ with probability at least $1-\delta$. This matrix can be applied to tensors $x^{(1)}\otimes\dots\otimes x^{(c)}\in R^{d^c}$ in $O(c\, m \min\{d,m\})$ time -- hence the name "Tensor Sketch". (Here $x\otimes y = \text{asvec}(xy^T) = [x_1y_1, x_1y_2,\dots,x_1y_m,x_2y_1,\dots,x_ny_m]\in R^{nm}$.) This improves upon earlier Tensor Sketch constructions by Pagh and Pham~[TOCT 2013, SIGKDD 2013] and Avron et al.~[NIPS 2014] which require $m=\Omega(3^c\lambda^2\delta^{-1})$ rows for the same guarantees. The factors of $\lambda$, $\varepsilon^{-2}$ and $\log1/\delta$ can all be shown to be necessary making our sketch optimal up to log factors. With another construction we get $\lambda$ times more rows $m=\tilde O(c\,\lambda^2\,\varepsilon^{-2}(\log1/\delta)^3)$, but the matrix can be applied to any vector $x^{(1)}\otimes\dots\otimes x^{(c)}\in R^{d^c}$ in just $\tilde O(c\, (d+m))$ time. This matches the application time of Tensor Sketch while still improving the exponential dependencies in $c$ and $\log1/\delta$. Technically, we show two main lemmas: (1) For many Johnson Lindenstrauss (JL) constructions, if $Q,Q'\in R^{m\times d}$ are independent JL matrices, the element-wise product $Qx \circ Q'y$ equals $M(x\otimes y)$ for some $M\in R^{m\times d^2}$ which is itself a JL matrix. (2) If $M^{(i)}\in R^{m\times md}$ are independent JL matrices, then $M^{(1)}(x \otimes (M^{(2)}y \otimes \dots)) = M(x\otimes y\otimes \dots)$ for some $M\in R^{m\times d^c}$ which is itself a JL matrix. Combining these two results give an efficient sketch for tensors of any size.

==> sections/notation_old <==


\begin{description}[leftmargin=!, labelwidth=5cm]
   \item[Kronecker product]
      $
      A\otimes B = 
      \begin{bmatrix}
         A_{1,1} B & \cdots & A_{1,n}B \\
         \vdots & \ddots & \vdots \\
         A_{m,1} B & \cdots & A_{m,n} B
      \end{bmatrix}
      $
   \item[Kronecker product (vectors)]
             $x \otimes y = 
             [x_1y_1, x_1y_2,\dots x_1y_m,\dots x_ny_m]^T$
\end{description}
\begin{center}
   \begin{tabular}{ l|l|l }
      name & notation & meaning
      \\
      %\hline
      Kronecker product
             & $A \otimes B$
             &
               $
                  \begin{bmatrix}
                     A_{1,1} B & \cdots & A_{1,n}B \\
                     \vdots & \ddots & \vdots \\
                     A_{m,1} B & \cdots & A_{m,n} B
                  \end{bmatrix}
               $
      \\
      Kronecker product (vectors)
             & $x \otimes y$
             & $[x_1y_1, x_1y_2,\dots x_1y_m,\dots x_ny_m]^T$
             %& $\asvec(x y^T)$
      \\
      Tensor power
             & $x^{\otimes k}$
             & $x \otimes x^{\otimes k-1}$
      \\
      Face-splitting product
             & $C \bullet D$
             &
               $
                  \begin{bmatrix}
                  C_1 \otimes D_1\\
                  \vdots\\
                  C_n \otimes D_n
                  \end{bmatrix}
               $
      \\
      Hadamard Porduct
             & $x \circ y$
             & $[x_1y_1, x_2y_2, \dots x_ny_n]^T$
   \end{tabular}
\end{center}


